Robustness of Safety for Linear Dynamical Systems: Symbolic and Numerical Approaches

In this paper, we study the robustness of safety properties of a linear dynamical system with respect to model uncertainties. Our paper involves three parts. In the first part, we provide symbolic (analytical) and numerical (representation based) techniques for computing the reachable set of uncertain linear systems. We further prove a relationship between the reachable set of a linear uncertain system and the maximum singular value of the uncertain dynamics matrix. Finally, we propose two heuristics to compute the robustness threshold of the system -- the maximum uncertainty that can be introduced to the system without violating the safety property. We evaluate the reachable set computation techniques, effects of singular values, and estimation of robustness threshold on two case studies from varied domains, illustrating the applicability, practicality and scalability of the artifacts, proposed in this paper, on real-world examples. We further evaluate our artifacts on several linear dynamical system benchmarks. To the best of the authors' knowledge, this is the first work to: (i) extend perturbation theory to compute reachable sets of linear uncertain systems, (ii) leverage the relationship between the reachable set of a linear system and the maximum singular values to determine the effect of uncertainties and (3) estimate the threshold of robustness that can be tolerated by the system while remaining safe.

==> extras.tex <==
\section{Extras}


==> introduction.tex <==
% \section{Introduction}
% \label{sec:intro}

\vspace{1ex}
\noindent \textbf{{\large Contributions:}}
In this section, we briefly introduce the main contributions of this paper: 
%
(i) A symbolic approach, using classical approaches from perturbation theory, to compute reachable sets of linear uncertain systems. In the previous works on uncertain linear systems, extensions of earlier proposed perturbation theory based methods have not been considered. To the best of the authors' knowledge, this is the first work to extend perturbation theory to compute reachable sets of linear uncertain systems.
%
Given a continuous time linear system $\dot x=A x$, and an initial set $\theta$, the reachable set at time $t$ is given by $\texttt{RS}_{\theta}(A,t)$ = $e^{At} \theta_0$. But, if there is some perturbation $E \in \mathbb{R}^{n \times n}$ introduced to the system, $i.e.$, the system now becomes $\dot x=(A+E) x$, the reachable set $\texttt{RS}_{\theta}(A,t)$ becomes invalid, and the computation of $e^{(A+E)t}$ needs to be performed from scratch to get the reachable set of the perturbed system.
% %
In \cite{kaagstrom1977bounds} and \cite{10.2307/2156675}, closed form upper bounds on the sensitivity of matrix exponential to such perturbations are given. Given $A$, $E$ $\in \mathbb{R}^{n \times n}$, closed form upper bound $\phi_{A,E}(t)$ is computed. This $\emph{relative error bound}$ $\phi_{A,E}(t)$ can be used as a \emph{bloating factor} for $\texttt{RS}_{\theta}(A,t)$ to compute the reachable set of $\dot x=(A+E) x$, without the need to compute $e^{(A+E)t}$ from scratch.
% %
In this work, we define linear uncertain systems as $\dot x=(A+\Lambda)x$, where $\Lambda \subset \mathbb{R}^{n \times n}$ is an interval matrix. Therefore, to use the idea described above, we use the results from \cite{farhadsefat2011norms} on interval matrices and extend the results of \cite{kaagstrom1977bounds} and \cite{10.2307/2156675} on closed form upper bounds of $\phi_{A,E}(t)$ to interval matrices, $i.e.$, $\phi_{A,\Lambda}(t)$. This approach is discussed in Section \ref{sec:perturbation}.
%
%
(ii) A set-based (numeric) approach to compute reachable sets of linear uncertain systems. For discrete time linear systems, the reachable set can be computed as a Minkowski sum of its autonomous part and the effect of the input (or perturbation) (\cite{girard2006efficient} and \cite{bak2017simulation}). If at a time step $k$, the reachable set of the autonomous part and the effect of input is $\Omega_k$ and $U_k$ respectively, then the cumulative reachable set of the system, at time step $k$, is given by $\Omega_k \oplus U_k$. We use this property of linear systems to compute the reachable set of a linear uncertain system. 
% %
Finally, we propose two methods to improve the performance of this approach. We discuss the details of this technique in Section \ref{sec:setBased}.
%
%
% The symbolic method, proposed in this paper, is computationally very efficient, but it considers a continuous dynamics. Whereas, the set based method discretizes the system and therefore able to compute reachable sets for a (given) particular time step.
% %
% Also, the set-based method does not require any template `shape' (for a polytopic representation)  to be provided, it determines a `shape' at every time step, represented as a generalized star ~\cite{bak2017hylaa}.
%
(iii) Prove a relationship between the reachable set of a linear uncertain system and the maximum singular value of the uncertain dynamics. 
%
To the best of the authors' knowledge, this is the first work to establish such a relationship. 
%
Leveraging this relationship, we propose two more useful artifacts that provide further insights to the behavior of linear uncertain systems: firstly, an algorithm to order the cells of the dynamics matrix based on its sensitivity to perturbation with respect to reachable sets; secondly, two heuristics to compute \textit{robustness threshold}.
%
Informally, given a nominal system $\dot{x}=Ax$ and an unsafe set $\mathcal{U}$, the \textit{robustness threshold} is defined as the perturbation $\Lambda$, \textit{s.t}, the reachable set of the system $\dot{x}=(A+\Lambda)x$ does not intersect with the unsafe set $\mathcal{U}$, \textit{i.e.}, the nominal system does not violate safety after the introduced perturbation. 


% Given a linear system $\dot{x}=A x$, an initial set $\theta$, time $t$: the reachable set is denoted as $\texttt{RS}_{\theta}(A,t)$.
% %
% We overload this operator to denote the reachable set of a linear uncertain system $\dot{x}=\Lambda_u x$ as $\texttt{RS}_{\theta}(\Lambda_u,t)$. 

% \textbf{Perturbation Analysis based approach (Symbolic)}. Given a continuous time linear system $\dot x=A x$, and an initial set $\theta$, the reachable set at time $t$ is given by $\texttt{RS}_{\theta}(A,t)$ = $e^{At} \theta_0$. But, if there is some perturbation $E \in \mathbb{R}^{n \times n}$ introduced to the system, $i.e.$, the system now becomes $\dot x=(A+E) x$, the reachable set $\texttt{RS}_{\theta}(A,t)$ becomes invalid, and the computation of $e^{(A+E)t}$ needs to be performed from scratch to get the reachable set of the perturbed system.
% %
% In \cite{kaagstrom1977bounds} and \cite{10.2307/2156675}, closed form upper bounds on the sensitivity of matrix exponential to such perturbations are given. Given $A$, $E$ $\in \mathbb{R}^{n \times n}$, closed form upper bound $\phi_{A,E}(t)$ is computed. This $\emph{relative error bound}$ $\phi_{A,E}(t)$ can be used as a \emph{bloating factor} for $\texttt{RS}_{\theta}(A,t)$ to compute the reachable set of $\dot x=(A+E) x$, without the need to compute $e^{(A+E)t}$ from scratch.
% %
% In this work, we define linear uncertain systems as $\dot x=(A+\Lambda)x$, where $\Lambda \subset \mathbb{R}^{n \times n}$ is an interval matrix. Therefore, to use the idea described above, we use the results from \cite{farhadsefat2011norms} on interval matrices and extend the results of \cite{kaagstrom1977bounds} and \cite{10.2307/2156675} on closed form upper bounds of $\phi_{A,E}(t)$ to interval matrices, $i.e.$, $\phi_{A,\Lambda}(t)$. This approach is discussed in Section \ref{sec:perturbation}.

% \textbf{Set-based approach (Numeric)}. 
% %
% For discrete time linear systems, the reachable set can be computed as a Minkowski sum of its autonomous part and the effect of the input (or perturbation) (\cite{girard2006efficient} and \cite{bak2017simulation}). If at a time step $k$, the reachable set of the autonomous part and the effect of input is $\Omega_k$ and $U_k$ respectively, then the cumulative reachable set of the system, at time step $k$, is given by $\Omega_k \oplus U_k$. We use this property of linear systems to compute the reachable set of a linear uncertain system. 
% %
% Given a continuous time linear uncertain system $\dot{x}=(A+\Lambda)x$, we perform the following steps:
% %
% (i) discretize the system, (ii) the reachable set at time step $k$ of the nominal dynamics $A$ is computed separately, and then added in Minkowski sense with the reachable set resulting from the perturbation $\Lambda$. 
% %
% Finally, we propose two methods to improve the performance of this approach. We discuss the details of this technique in Section \ref{sec:setBased}.

% \textbf{Classifying Uncertainties}. 
% Given a linear uncertain system $x^+=(A+\Lambda)x$, equivalently, $x^+=\Lambda_ux$, where $\Lambda_u=A+\Lambda$: we prove a relationship between the reachable set of the linear uncertain system and the maximum singular value of the uncertain dynamics matrix $\Lambda_u$. Informally, the relationship states that the reachable set of the linear uncertain system is dictated by the maximum singular value of the uncertain dynamics matrix, \textit{i.e.}, the reachable set can computed very efficiently as a function of just the maximum singular value of $\Lambda_u$, for a special case. The proof, establishing the relationship, is provided in Subsection \ref{subsec:2xProof}. Using the fact that the maximum singular value of the uncertain dynamics matrix dictates the reachable set of the uncertain system, we provide an algorithm to order the cells of the nominal matrix $A$, based on its sensitivity to perturbation. The intuitive idea of the ordering algorithm is as follows:  if a cell $(i,j)$ of $A$ has more impact than a cell ($k,l)$ on the maximum singular value, then $(k,l)$ is more tolerant to perturbation than $(i,j)$. Using this idea and the results from \cite{it:1999-001}, we propose an algorithm to provide an ordering on the cells of the matrix $A$, based on its sensitivity to perturbation. The details of the ordering algorithm is provided in Subsection \ref{subsec:ordering}. Finally, leveraging the ordering algorithm, we provide two heuristics to compute the robustness threshold of the system. Given $x^+=Ax$ and an unsafe set, we compute a $\Lambda_{R}$, \textit{s.t}, the system $x^+=(A+\Lambda_{R})x$ is safe. The two heuristics, mentioned in this paper, computes $\Lambda_{R}$ iteratively by introducing small fractions of a perturbation to the cells of $A$ that are less tolerant to perturbation (as computed by the ordering algorithm), and higher fractions of the perturbation are introduced to the cells of $A$ that are more tolerant to perturbations. The iteration continues by increasing the the the total amount of perturbation at each step, until the system $x^+=A+\Lambda_{R}x$ becomes unsafe, \textit{i.e.}, the last $\Lambda_{R}$ for which the system $x^+=A+\Lambda_{R}x$ is safe, is returned as the robustness threshold of the system.

This paper is organized as follows.
%
In Section \ref{sec:prelims}, we provide the notations and the formal definitions that has been used in the rest of the paper.
%
In Section \ref{sec:perturbation}, we discuss the symbolic approach to compute reachable sets of linear uncertain systems.
%
In Section \ref{sec:setBased}, we discuss the set-based approach, along with its performance improving techniques to compute reachable sets of linear uncertain systems.
%
In Section \ref{sec:uncertainties}, we prove the relationship between the reachable set of linear uncertain systems and the maximum singular value of the uncertain dynamics matrix. We further provide an algorithm to order the cells of the nominal dynamics matrix, and two heuristics to compute robustness threshold.
%
In Section \ref{sec:evaluation}, we provide an extensive evaluation of all the aforementioned techniques on several low to high dimensional benchmarks.
%
We finally conclude our work in Section \ref{sec:conclusion}.


==> motivation_relatedWork.tex <==
\section{Motivation and Related Work}
\label{sec:motivation_relatedWork}
Safety analysis of cyber-physical systems require a precise mathematical model of the system. 
%
Since constructing a precise model is subjected to measurement and sensor uncertainties, it is important to understand the robustness of the safety analysis, \textit{i.e.}, whether the safety specification holds true for some perturbations in the model.
%
For safety critical systems, understanding robustness of safety analysis is even more essential.

A (continuous time) linear dynamical system without uncertainties is defined as $\dot{x}=Ax$, where the the dynamics matrix $A$ is assumed to be known accurately, $i.e.$, all the elements of the matrix are known accurately. 
%
Consider the following Example \ref{ex:linearSys} of a linear system.
%
\begin{example}
\label{ex:linearSys}
Consider the continuous time linear dynamical system $\dot{x} = Ax$, where $A$ is 
$
\begin{bmatrix}
    1  & c \\
    0  & 2 
\end{bmatrix}
$
and $c$ represents a system parameter.
\end{example}
%
Traditional methods of reachable set computation of linear systems assume a fixed value of $c$ (say, -1).
%
But in reality, the value of $c$ is not known exactly, instead, it is only estimated. Therefore, considering the sensing and actuation uncertainties, one should think of the value as a parameter that can take a range of values  \big(say, $a \in [-1.1,-0.9]$\big).
%
Often, the safety proofs provided using reachable set based techniques cannot account for such uncertainties.
%
Further, the reachable set techniques do not inform us about the amount of uncertainties that can be tolerated while maintaining safety.

% Such reachable sets that does not account for uncertainties, when used to perform safety analysis could result in fatal mistakes. 
% %
% For the reachable sets to be sound in safety analysis, it must consider the effect of uncertainties in the model. 

In this paper, we consider a model with uncertainties --- we define continuous time linear uncertain systems as $\dot{x}=\Lambda_u x$ (corresponding discrete time uncertain system is defined in \cite{10.1145/3358229}), where the uncertainties in the model are considered as variables in $\Lambda_u$ that can take values from a bounded range. 
%
% For instance, in Example \ref{ex:linearSys}, instead of assuming $a$ as 9.8, $a$ is a variable in $\Lambda_u$ and all other entries in $\Lambda_u$ are same as $A$. 
%
Interval matrix, a matrix where intervals as elements is a convenient representation of such a matrix $\Lambda_u$.
% can also be represented as an interval matrix.
%
The linear uncertain system $\dot{x}=\Lambda_u x$ can equivalently be represented by separating the nominal and the perturbed dynamics as $\dot{x}=(A+\Lambda) x$, where $\Lambda_u=A+\Lambda$.
%

Our goal in this paper is to determine the uncertainties $\Lambda$ can be tolerated by the matrix $A$ without violating the safety property.
%
We call it the \emph{robustness threshold}.
%
For computing this, we propose a symbolic and a set-based (numeric) method to compute reachable sets that take into account the effect of uncertainties.
%
Second, we demonstrate the relationship between uncertainties and reachable set using the maximum singular values.
%
Finally, we propose two heuristics to compute the robustness threshold.
% 
% Further, we provide several other artifacts that provide more understanding on types and effects of various classes of uncertainties on a linear system (discussed later).

\vspace{1ex}
\noindent \textbf{{\large Related Work:}} In the rest of this section, we discuss the techniques for computing reachable sets of linear uncertain systems available in the literature.
%
In \cite{10.1145/3358229}, a class of uncertainties are identified by a set of sufficient conditions on the structure of the dynamics matrix $\Lambda_u$. 
%
For such classes of uncertainties, the exact reachable set of the linear dynamical system can be computed very efficiently.
%
Unfortunately, this technique is unable to handle arbitrary set of uncertainties.
% 
In \cite{DBLP:conf/emsoft/LalP15}, given a linear uncertain system $\dot{x}=\Lambda_u x$, where there are parametric uncertainties in $\Lambda_u$; the authors' provide a sampling interval $\delta>0$, given an $\epsilon>0$, $s.t.$, the piecewise bilinear function, approximating the solution by interpolating at these sample values, is within $\epsilon$ of the original trajectory.
%
In \cite{althoff2011reachable}, given a continuous time linear system with input, the system is discretized and reachable set for consecutive time intervals are computed. 
%
For a given time step, the reachable set is computed in three steps: 
%
(i) the reachable set ignoring the input is computed; 
%
(ii) generate the convex hull of the solution at that time step and the initial set; 
%
(iii) enlarge the convex hull to ensure enclosure of all trajectories for the time interval, including the effects of inputs. 
%
It uses \emph{Peano-Baker} series to compute an over-approximation of reachable set. 
%
In \cite{COMBASTEL20114525}, the authors provide an algorithm for computation of envelopes enclosing the possible states and/or outputs of a class of linear uncertain systems. 
%
It extends an existing algorithm based on Zonotopes, so that it can efficiently propagate structured parametric uncertainties. 
%
Note that this work can handle only a class of uncertainties, but unlike \cite{10.1145/3358229}, they don't provide an exact reachable set --- the over-approximate flow-pipe has been empirically shown to handle the wrapping effect (\emph{i.e.} the tightness of over-approximation).

Unlike all these works mentioned, we propose: 
%
(i) A symbolic approach, using classical approaches from perturbation theory, which is computationally very fast.
%
(ii) A set based representation (numeric) approach, where the reachable set is represented as a Minkowski sum of its unperturbed part with the effect of perturbation. 
%
Unlike \cite{althoff2011reachable}, which uses \emph{Peano-Baker} series to compute an over-approximation of reachable set, our (set-based) approach of discretizing the system is different. 
%
Moreover, we use generalized stars \cite{duggirala2016parsimonious} to represent our sets and compute an over-approximation of the reachable set to account for uncertainties using the generalized stars.
%
We also provide two methods to improve the performance of our set based representation method.
%
(iii) We provide several other artifacts that provide more understanding on types and effects of various classes of uncertainties on a linear system.
